Turchin's Relation for Call-by-Name Computations: A Formal Approach

Supercompilation is a program transformation technique that was first described by V. F. Turchin in the 1970s. In supercompilation, Turchin's relation as a similarity relation on call-stack configurations is used both for call-by-value and call-by-name semantics to terminate unfolding of the program being transformed. In this paper, we give a formal grammar model of call-by-name stack behaviour. We classify the model in terms of the Chomsky hierarchy and then formally prove that Turchin's relation can terminate all computations generated by the model.

==> eptcsdata.tex <==
\providecommand{\firstpage}{137}
\providecommand{\publicationstatus}{G.W. Hamilton, A. Lisitsa, A.P. Nemytykh (Eds): VPT 2016\\
EPTCS 216, 2016, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.216.8}{10.4204/EPTCS.216.8}}
\pdfoutput=1

